Deep Thermal Infrared Imaging of HR 8799 bcde: New Atmospheric Constraints and Limits on a Fifth Planet

We present new $L^\prime$ (3.8 $\mu m$) and Br-$\alpha$ (4.05 $\mu m$) data and reprocessed archival $L^\prime$ data for the young, planet-hosting star HR 8799 obtained with Keck/NIRC2, VLT/NaCo and Subaru/IRCS. We detect all four HR 8799 planets in each dataset at a moderate to high signal-to-noise (SNR $\gtrsim$ 6-15). We fail to identify a fifth planet, "HR 8799 f", at $r$ $<$ 15 $AU$ at a 5-$\sigma$ confidence level: one suggestive, marginally significant residual at 0.2" is most likely a PSF artifact. Assuming companion ages of 30 $Myr$ and the Baraffe (Spiegel \& Burrows) planet cooling models, we rule out an HR 8799 f with mass of 5 $M_{J}$ (7 $M_{J}$), 7 $M_{J}$ (10 $M_{J}$), and 12 $M_{J}$ (13 $M_{J}$) at $r_{proj}$ $\sim$ 12 $AU$, 9 $AU$, and 5 $AU$, respectively. All four HR 8799 planets have red early T dwarf-like $L^\prime$ - [4.05] colors, suggesting that their SEDs peak in between the $L^\prime$ and $M^\prime$ broadband filters. We find no statistically significant difference in HR 8799 cde's colors. Atmosphere models assuming thick, patchy clouds appear to better match HR 8799 bcde's photometry than models assuming a uniform cloud layer. While non-equilibrium carbon chemistry is required to explain HR 8799 bc's photometry/spectra, evidence for it from HR 8799 de's photometry is weaker. Future, deep IR spectroscopy/spectrophotometry with the Gemini Planet Imager, SCExAO/CHARIS, and other facilities may clarify whether the planets are chemically similar or heterogeneous.

==> tab_phothr8799.tex <==
\begin{deluxetable}{llcllccccccc}
\setlength{\tabcolsep}{0pt}
\tablecolumns{8}
\tablecaption{$\beta$ Pictoris b Detections and Photometry}
\tiny
\tablehead{{UT Date}&{Telescope/Instrument }&{ Filter }&{ Wavelength ($\mu m$)}&{ SNR }&{ Apparent Magnitude } &{Absolute Magnitude}}
\startdata
2011-12-16&VLT/NaCo & J & 1.25 & 9.2 & 14.11 $\pm$ 0.21 & 12.68 $\pm$ 0.21\\
2012-01-01&VLT/NaCo & H & 1.65 & 30 & 13.32 $\pm$ 0.14 & 11.89 $\pm$ 0.14\\
\\
2013-01-09&Gemini/NICI & H & 1.65 & 6.4 & 13.25 $\pm$ 0.18 & 11.82 $\pm$ 0.18\\
2013-01-09&Gemini/NICI & K$_{s}$ & 2.16 & 10 & 12.47 $\pm$ 0.13 & 11.04 $\pm$ 0.13\\
%VLT/NaCo &  K$_{s}$ & 2.18 & 8 & xxx $\pm$ 0.13 & xxx\\
%2012-12-23&Gemini/NICI& [3.09] & 3.09 & 11 & 11.36 $\pm$ 0.5 & 9.93 $\pm$ 0.5\\
2012-12-23&Gemini/NICI& [3.09] & 3.09 & 4.6 & 11.71 $\pm$ 0.27 & 10.28 $\pm$ 0.27\\
2012-12-26&Gemini/NICI& [3.09] & 3.09 & 11 & -- & --\\
%Gemini/NICI & L$^\prime$ & 3.78 & 9 & xxx$\pm$ xxx & xxx\\
\\
2012-12-16&VLT/NaCo &  L$^\prime$ & 3.8 & 40 & 11.24 $\pm$ 0.08 & 9.81 $\pm$ 0.08\\
2012-12-16&VLT/NaCo &  [4.05] & 4.05& 20 & 11.04 $\pm$ 0.08 & 9.61 $\pm$ 0.08\\
2012-12-15&VLT/NaCo & M$^\prime$ & 4.78& 22 & 10.96 $\pm$ 0.13 & 9.54 $\pm$ 0.13\\
 \enddata
%\tablecomments{}
\label{bpicphot}
\end{deluxetable}

